Accurate Learning or Fast Mixing? Dynamic Adaptability of Caching Algorithms

Typical analysis of content caching algorithms using the metric of steady state hit probability under a stationary request process does not account for performance loss under a variable request arrival process. In this work, we consider adaptability of caching algorithms from two perspectives: (a) the accuracy of learning a fixed popularity distribution, and (b) the speed of learning items' popularity. In order to attain this goal, we compute the distance between the stationary distributions of several popular algorithms with that of a genie-aided algorithm that has knowledge of the true popularity ranking, which we use as a measure of learning accuracy. We then characterize the mixing time of each algorithm, i.e., the time needed to attain the stationary distribution, which we use as a measure of learning efficiency. We merge both measures above to obtain the "learning error" representing both how quickly and how accurately an algorithm learns the optimal caching distribution, and use this to determine the trade-off between these two objectives of many popular caching algorithms. Informed by the results of our analysis, we propose a novel hybrid algorithm, Adaptive-LRU (A-LRU), that learns both faster and better the changes in the popularity. We show numerically that it also outperforms all other candidate algorithms when confronted with either a dynamically changing synthetic request process or using real world traces.

==> 08B2-partitions.tex <==

%\subsection{Effective Hit Probability of Linear Caching Algorithms over Partitions}
\subsubsection{Impact of Cache Partitions: LRU($\boldsymbol m$) vs. LRU}
\blue{Numerical experiments were also conducted for a large linear cache network, where the tuple $(n, m)$ is comparable to real cache networks.  We illustrate how different algorithms perform using a content library size of $n=3,000$ with sufficiently long runs (i.e., enough number of requests to make sure that the system has reach steady state, e.g., about $6\times 10^6$ requests).  The hit probability of the algorithms are calculated as $\text{Hit probability}={\text{Total No. of Hit Counts}}/{\text{Total No. of Request Counts}}$.}

\blue{We first study how hit probability varies with the total cache size and the number of cache levels.  Figure~\ref{fig:syn-sim1-lru} shows the hit probabilities achieved by LRU($\boldsymbol m$), where  we assume that $m_{i+1}=0.5m_i$ for $i=2, \cdots, h$, satisfying $\sum_{i=1}^h m_i=m.$  The hit probabilities increase with total cache size $m,$ as well as the number of caches in the linear cache network.  However, the gain becomes limited when $h\geq 5$.  In other words, most caching gain can be obtained by using a small number of cache levels.}  

\blue{We next consider the impact of the cache partitioning policy on performance.  In particular, we focus on the division between cache $1$ and all the others.  Hence, we vary $m_1$ and divide the remaining cache size evenly among the remaining $h-1$ caches, given a fixed total cache size $m=900.$   Figure~\ref{fig:syn-sim2-lru} shows the hit probabilities of LRU($\boldsymbol m$) as a function of the cache partitions (decreasing value of $m_1$).  We see that the hit probability increases as the higher level caches are assigned more space.  In summary, the hit probability of a caching policy increases by favoring more levels and assigning more resources to higher level caches.}


\blue{From the mixing time analysis in Section~\ref{sec:lru-m-mixing}, we also consider the two extreme cases: Case $1$ with $m_1=\cdots=m_{h-1}=1,$ $m_h=m-h+1$ and Case $2$ with $m_1=m-h+1$, $m_2=\cdots=m_h=1,$ and make a comparison with the upper envelope of achievable hit probability by LRU($\boldsymbol m$), which we call it Case $3.$ The results are shown in Figure~\ref{fig:hit-prob-time-multi-partitions} with $(n, m)=(100, 15)$. We observe that allocating more cache capacity to higher level caches improve the hit probability at the cost of longer learning time, which is consistent with the mixing time analysis in Section~\ref{sec:lru-m-mixing}. }

